Analysis of Bootstrap and Subsampling in High-dimensional Regularized Regression

We investigate popular resampling methods for estimating the uncertainty of statistical models, such as subsampling, bootstrap and the jackknife, and their performance in high-dimensional supervised regression tasks. We provide a tight asymptotic description of the biases and variances estimated by these methods in the context of generalized linear models, such as ridge and logistic regression, taking the limit where the number of samples $n$ and dimension $d$ of the covariates grow at a comparable fixed rate $\alpha\!=\! n/d$. Our findings are three-fold: i) resampling methods are fraught with problems in high dimensions and exhibit the double-descent-like behavior typical of these situations; ii) only when $\alpha$ is large enough do they provide consistent and reliable error estimations (we give convergence rates); iii) in the over-parametrized regime $\alpha\!<\!1$ relevant to modern machine learning practice, their predictions are not consistent, even with optimal regularization.

==> Figures/logistic/lambda=0.01/logistic_regression_lambda=0.01_bias.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\tikzstyle{every node}=[font=\scriptsize]
\begin{axis}[
width=\figwidth,
height=\figheight,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={\(\displaystyle n / d\)},
xmajorgrids,
xmin=0.025, xmax=10.475,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Bias},
ymajorgrids,
ymin=0.000465908987369071, ymax=6.88981009775995,
ymode=log,
ytick style={color=black}
]
\addplot [semithick, black]
table {%
0.5 0.115406438884387
0.75 0.000720845642193879
1 0.0771736188332288
1.25 0.322075814664895
1.5 0.67184348607442
1.75 0.963612323894962
2 0.99375835180983
2.25 0.813446942503774
2.5 0.605185539530038
2.75 0.444413700376856
3 0.331691110612977
3.25 0.254029769204307
3.5 0.200077835427657
3.75 0.161180657744752
4 0.132379634327751
4.25 0.110513740016192
4.5 0.0939004830995707
4.75 0.0804733833380262
5 0.0699487130377587
5.25 0.0611162800209866
5.5 0.054059829945158
5.75 0.0481517626167971
6 0.04296898596992
6.25 0.0387503255959096
6.5 0.0351211595108514
6.75 0.0319772450012006
7 0.0290760880840453
7.25 0.0266982989445141
7.5 0.0245996679595231
7.75 0.0227383633793612
8 0.0210800576689731
8.25 0.0195963757963962
8.5 0.0181300655588377
8.75 0.0169445897749716
9 0.0158713323947248
9.25 0.0148966200674217
9.5 0.0140087911059084
9.75 0.0131978522202885
10 0.0124551991283939
};
\addlegendentry{$\biasOnXY$}
\addplot [semithick, red, dashed]
table {%
0.5 0.918701630659635
0.75 1.69104663083934
1 2.65698825068402
1.25 3.71235026870671
1.5 4.45313706280153
1.75 4.11465597764212
2 2.42889453096387
2.25 0.998109656658642
2.5 0.839872478950557
2.75 1.10948421756716
3 1.8377004516389
3.25 2.00075160530039
3.5 1.81555010369927
3.75 1.52022897544038
4 1.24167278268356
4.25 0.862681227146082
4.5 0.74336940833086
4.75 0.590725971572219
5 0.46358623937352
5.25 0.371784750413235
5.5 0.302507186462039
5.75 0.248913424117251
6 0.208199960412044
6.25 0.174908588059402
6.5 0.159910000850146
6.75 0.138279150923927
7 0.117305400510069
7.25 0.102721242582264
7.5 0.091875763147387
7.75 0.0786883878157925
8 0.0701457358622468
8.25 0.0627288643671493
8.5 0.0539247295102303
8.75 0.0486242928089737
9 0.0440055692143915
9.25 0.0399261597266438
9.5 0.0350899066662285
9.75 0.0320265262853132
10 0.0292913473345537
};
\addlegendentry{$\biasPairBootstrap$}
\end{axis}

\end{tikzpicture}


==> Figures/logistic/lambda=1/logistic_regression_lambda=1.0_bias.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\tikzstyle{every node}=[font=\scriptsize]
\begin{axis}[
width=\figwidth,
height=\figheight,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={\(\displaystyle n / d\)},
xmajorgrids,
xmin=0.025, xmax=10.475,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Bias},
ymajorgrids,
ymin=1.19394824737162e-05, ymax=1.45057295746595,
ymode=log,
ytick style={color=black}
]
\addplot [semithick, black]
table {%
0.5 0.85196839151246
0.75 0.789506635505128
1 0.733402904145799
1.25 0.682921827168845
1.5 0.63734952970136
1.75 0.596089308199753
2 0.558621650684909
2.25 0.524526737681789
2.5 0.493415681220116
2.75 0.464956878225641
3 0.438857915716394
3.25 0.414862324125022
3.5 0.39278123835327
3.75 0.37240576195238
4 0.353568294239081
4.25 0.336117963181273
4.5 0.319921485756118
4.75 0.304869217762514
5 0.290853961284697
5.25 0.277783547738398
5.5 0.265575696406583
5.75 0.254156784041304
6 0.243460792592616
6.25 0.23342839544342
6.5 0.224006170639576
6.75 0.215145916770009
7 0.206804058989069
7.25 0.19894113241287
7.5 0.191521328334004
7.75 0.184510031651427
8 0.177881776373535
8.25 0.171607444039647
8.5 0.165662350829353
8.75 0.16002391630761
9 0.154671091582078
9.25 0.149585615298052
9.5 0.144749692403422
9.75 0.140147281230552
10 0.135763599689085
};
%\addlegendentry{erm bias}
\addplot [semithick, red, dashed]
table {%
0.5 0.00108510339623194
0.75 0.00136569297247272
1 0.00154908138760121
1.25 0.001714356676282
1.5 0.00176885657778425
1.75 0.00175224432331195
2 0.00171946376631021
2.25 0.00167199316057026
2.5 0.00157646672520972
2.75 0.00149468253302909
3 0.00141334096255663
3.25 0.00134499458444171
3.5 0.00125843075323662
3.75 0.00118509183952797
4 0.00110278517224138
4.25 0.00102651901582229
4.5 0.000952691701195607
4.75 0.000870641766370195
5 0.000799955025525545
5.25 0.000736974994930417
5.5 0.00067727739641843
5.75 0.000620770643274815
6 0.000567173398453691
6.25 0.000508133330279104
6.5 0.000459094094985679
6.75 -0.000169636068819257
7 -0.000124484025188165
7.25 -2.08414631013287e-05
7.5 6.57731398436834e-05
7.75 0.000139859238680984
8 0.000221381546422705
8.25 0.000309355755526042
8.5 0.000213454026446902
8.75 0.000158608052749143
9 0.000121725283736218
9.25 8.75893717362519e-05
9.5 5.37985018282949e-05
9.75 2.03283250588271e-05
10 -1.34449792070779e-05
};
%\addlegendentry{bootstrap bias estimation}
\end{axis}

\end{tikzpicture}

